LeakageDetector: An Open Source Data Leakage Analysis Tool in Machine Learning Pipelines

Code quality is of paramount importance in all types of software development settings. Our work seeks to enable Machine Learning (ML) engineers to write better code by helping them find and fix instances of Data Leakage in their models. Data Leakage often results from bad practices in writing ML code. As a result, the model effectively ''memorizes'' the data on which it trains, leading to an overly optimistic estimate of the model performance and an inability to make generalized predictions. ML developers must carefully separate their data into training, evaluation, and test sets to avoid introducing Data Leakage into their code. Training data should be used to train the model, evaluation data should be used to repeatedly confirm a model's accuracy, and test data should be used only once to determine the accuracy of a production-ready model. In this paper, we develop LEAKAGEDETECTOR, a Python plugin for the PyCharm IDE that identifies instances of Data Leakage in ML code and provides suggestions on how to remove the leakage.

==> Sections/02_Background.tex <==
\section{Related Work}
\label{Section:Background}




==> Sections/07_Threats.tex <==
%\vspace{-.2cm}
\section{Threats to Validity}
\label{Section:Threats}

In this section, we describe potential threats to the validity of our research method and the actions we took to mitigate them.





==> Sections/all.tex <==
\begin{abstract}
This paper presents a study that investigates the use of PMD, a static analysis tool, to identify and resolve bugs in open source projects using static analysis tools. The study was conducted in an educational environment using Java-based software projects with a number of problems. Students were asked about their attitudes towards utilizing ChatGPT in terms of a variety of aspects, including (1) the capability of ChatGPT to fix bugs, (2) the ability of ChatGPTt to introduce additional bugs by programming mode debugging (PMD), and (3) the frequency of interactions with ChatGPT for bug fixing purposes. Most students (96.8\%) expressed their acceptance to Gpt, admitting that it is indeed useful. It is. It highlights the importance of including other traditional static analysis tools and techniques to improve accuracy and effectiveness of their predictions. This study sheds some light on the feasibility of this learning activity for educating students to effectively review and control code.
\end{abstract}
\section{Related Work}
\label{Section:Background}
%\subsection{ChatGPT in SE tasks.} 
Recent studies utilized \gpt for different software engineering tasks. Due to the importance of the topic, several domains for using \gpt have been proposed including code quality \cite{white2023prompt,white2023chatgpt}, programming \cite{biswas2023role,sun2023automatic,tian2023chatgpt,liu2023your}, testing \cite{siddiq2023exploring}, bug management \cite{haque2023potential,sobania2023analysis,xia2023keep}, security \cite{khoury2023secure}, and program comprehension \cite{ma2023scope}.  In this section, we are only
interested in research on using \gpt to solve software engineering tasks, summarized in Table \ref{Table:chatgpt-relatedwork}.

White \etal \cite{white2023prompt,white2023chatgpt} presented prompt design techniques for software engineering using patterns to solve common problems when using large language models (LLMs). The study provides a catalog of patterns for software engineering that classifies patterns according to the types of problems they solve. Additionally, the authors explored several prompt patterns developed to improve code quality, refactoring, requirements elicitation, and software design. In another study, Biswas \cite{biswas2023role} discussed an overview of \gpt as a language model developed by OpenAI that offers a wide range of capabilities for computer programming. These capabilities include code completion, correction, prediction, error fixing, optimization, document generation, chatbot development, text-to-code generation, and technical query answering. The author highlighted the ability of \gpt to provide explanations and guidance to users and concluded that it is a powerful tool for the programming community. On the other hand, Siddiq \etal \cite{siddiq2023exploring} explored the effectiveness of LLMs in generating unit tests using two benchmarks: HumanEval and Evosuite.Their findings show that the generated tests also contains test smells such as Duplicated Asserts and Empty Tests. Sun \etal \cite{sun2023automatic} utilized \gpt to automate code summarization. The authors adopt widely-used metrics to assess the quality of the generated comments. The findings show that \gpt performs worse than SOTA models. Haque and Li \cite{haque2023potential} explored the capabilities of \gpt as a debugging tool and best practices for integrating it into the software development workflow. Their findings show that \gpt is  a helpful tool for debugging, but it  should  be  used  cautiously in software development. In another study, Sobania \etal \cite{sobania2023analysis} evaluated \gpt on standard bug fixing benchmark and compared its performance with Codex, CoCoNut, and APR. Compared to these approaches, \gpt fixes 31 out of 40 bugs, but the success rate can be further increased. To understand if \gpt is the ultimate programming assistant, Tian \etal \cite{tian2023chatgpt} empirically experimented by emphasizing three code-related tasks: code generation, code summarization and program repair. For code generation, \gpt struggles to generalize to new and unseen problems. For program repair, \gpt achieves competitive results compared to Refactory. For code summarization, \gpt may not be able to explain the intention of the given code samples accurately. Liu \etal \cite{liu2023your} answered the question on whether code generated by \gpt really correct. To do so, the authors combined LLM-based and mutation-based input generation to evaluate the correctness of LLM-generated code. In a security-related context, Khoury \etal \cite{khoury2023secure} investigated how secure the code generated by \gpt. Their results suggested that \gpt is aware of potential vulnerabilities but can generate code that lack robustness to certain attacks. Xia and Zhang \cite{xia2023keep} proposed ChatRepair to automate a conversation-driven automated program repair approach. The tool feeds the LLM with information on relevant test failures and then learns from failures and successes of earlier patching attempts of the same bug. Their tool achieved the new state-of-the-art in program repair performance. Ma \etal \cite{ma2023scope} performed a study evaluating \gpt capabilities and limitations in software engineering from three aspects: 1) syntax understanding, 2) static behavior understanding, and 3) dynamic behavior understanding. The authors concluded that \gpt
possesses capabilities akin to an Abstract Syntax Tree (AST)
parser, \gpt is susceptible
to hallucination when interpreting code semantic structures and
fabricating non-existent facts, which underscore the need
to explore methods for verifying the correctness of \gpt
outputs to ensure its dependability in software engineering tasks.

%%% PMD
\textcolor{black}{To summarize, the study of static analysis tools has been extensively studied (\eg \cite{romano2022static,liu2018mining,plosch2008relation}). Since we are focusing on Java,  there are a few widely adopted Java-based open-source static analysis tools such as CheckStyle\footnote{https://checkstyle.sourceforge.io}, FindBugs\footnote{http://findbugs.sourceforge.net}, JLint\footnote{http://jlint.sourceforge.net/}, PMD\footnote{https://pmd.sourceforge.io} and SonarQube\footnote{https://www.sonarqube.org/}. The choice of PMD is motivated by different factors:  its widespread use in the Java community and its maturity (\ie it has been available since 2002 and therefore has been in use for a long time \cite{trautsch2020longitudinal}), and works on the Java source code to find coding style problems, which is not the case by FindBugs and JLint that work on byte code and focus on finding programming errors and neglecting programming style issues \cite{plosch2008relation}. CheckStyle focuses more on readability problems compared to PMD, which tends to highlight suspicious situations in the source code \cite{panichella2015would}. Further, although there are recent studies that explored the use of static analysis tools on open-source communities focusing on how warnings evolve across the software evolution history \cite{trautsch2020longitudinal,di2009life,kim2007warnings}, \textcolor{black}{this is the first study investigating how \gpt can support students in improving code quality, and reflecting on how students are using it in the classroom.} To advance the understanding of learning how to find and fix bugs and whether \gpt eventually would be code companion or code replacement, in this paper, we performed a study in an educational setting using open-source projects with many issues. This study complements the existing efforts that are done in open source systems \cite{kim2007warnings,plosch2008relation,di2009life,panichella2015would,beller2016analyzing,singh2017evaluating,liu2018mining,digkas2018developers,querel2018warningsguru,marcilio2019static,aloraini2019empirical,trautsch2020longitudinal,romano2022static,licorish2022combining} and in education \cite{mengel1999case,edwards2019can,luukkainen2022aspa,senger2022helping,alomar2023use}, by complementing the quantitative analysis with a qualitative one, providing evidence of several kinds of warnings students pay more attention to, during code analysis.}
%\input{Tables/RelatedWork-pmd}
\input{Tables/RelatedWork-chatgpt}

%Since students are relying on \gpt, this motivated us to learn how to use it in our favor to help them with debugging process and whether this eventually replaces them in that process or not. 

%How we can use \gpt in the classroom and the limitation of LLMs. For educator, it helps them how to use \gpt in the classroom. Learning and adjusting work to take advantage of the good side of \gpt and learn the motivation.

%Students don't trust entirely \gpt and train them to critique and see how \gpt can miss up their code.


%\vspace{-.3cm}
\section{Study Design} \eman{TODO: add approach overview}
\label{Section:methodology}

\subsection{Goal \& Research Questions}
We formulate the main goal of our study based on the \textit{Goal} \textit{Question} \textit{Metric} template \cite{van2002goal}, as follows:

\begin{figure*}[t]%[H]
 	\centering
 	\includegraphics[width=1.0\textwidth]{Images/ChatGPT.pdf}
 	\caption{Key phases of our study.}
 	\label{fig:approach}
%\vspace{-.4cm}
\end{figure*}
\begin{tcolorbox}
\textit{\textbf{Analyze} the use of \gpt \textbf{for the purpose of} \textcolor{black}{familiarizing students with improving source code, by developing the culture of reviewing unknown code and patching it} \textit{with respect to} software quality \textbf{from the point view} of educators \textbf{in the context of} undergraduate and graduate students in SE/CS who analyze Java-based software projects.}
\end{tcolorbox}

According to our goal, we aim to answer the following research questions:

\begin{itemize}
\item \textbf{RQ1. \textit{\RQone}}

\underline{Motivation:} \textcolor{black}{This RQ aims at evaluating whether students can apply analytical skills to identify and fix issues in existing systems. The findings will shed some light on the feasibility of this learning activity to educate students to perform effective code reviews and quality control.}

\underline{Measurement:} \textcolor{black}{We examine (1) the types of issues that can be identified and  (2) the PMD ruleset categories that are selected by students.} 

\item \textbf{RQ2. \textit{\RQtwo}}

\underline{Motivation:} \textcolor{black}{This RQ investigates which PMD ruleset is taking longer time to be fixed by ChatGPT, with respect to other rulesets. The finding raises educators' awareness of issues types that are hard for students to understand and address.} %the challenges students faced when performing code reviews using ASAT.

\underline{Measurement:} \textcolor{black}{We examine the resolution time taken by students to fix each ruleset, clustered by category.}


\item \textbf{RQ3. \textit{\RQthree}}

\underline{Motivation:} \textcolor{black}{This RQ explores the tool's feedback, and how students perceive \gpt in general. The finding will inform educators on the usefulness, usability, and functionality of the tool, and allow them to make decisions about how \gpt can better support students with code improvement.}

\underline{Measurement:} \textcolor{black}{We examine students' feedback. We extract all their positive and negative comments as they describe their experience using ChatGPT.}

\end{itemize}
 
 \textcolor{black}{As part of this paper’s contributions, we provide the assignment description, dataset, and tool documentation for educators to adopt and extend}\footnote{XXX}. 

 \subsection{Course Overview}

\hl{Software quality assurance is a graduate course}, consisting of 2 lectures weekly, an hour and 15 minutes each. The course explores the foundations of software quality and maintenance and introduces challenges linked to various aspects of software evolution, along with support tools to approach them. Also, the course covers various concepts related to software analysis and testing, along with practical tools widely used as industry standards. Students were also given several hands-on assignments on software quality metrics, code refactoring, bug reporting, unit and mutation testing, and technical debt management. The course deliverables consisted of five individual homework assignments, a research paper reading and presentation, and a long-term group project.

\subsection{Teaching Context and Participants}

The study involves one assignment in the software quality assurance course. The course was taught at \hl{X} and \hl{X} for 3 semesters. Before conducting the assignment, students have already learned about several code, and design quality concerns: (1) code quality (teaching quality concepts and how to measure software quality), (2) code smells (teaching bad programming practices that violate design principles), (3) code refactoring (teaching refactoring recipes that help improving software quality), and (4) bug management (teaching software bugs and how to locate and fix them). The assignment constituted 7.5\% of the final grade. It was due 14 days after the four corresponding sessions. 

\textcolor{blue}{In Spring semester, \hl{X} students registered to this course. In total, \hl{X} students completed the assignment and participated in the questionnaire. Participation in the survey was voluntary. No extra grades or other types of benefits were provided to the students who completed the survey. The programming experience of the
respondents ranged from 1 to more than 10 years, their Java 
experience ranged from 1 to 10 years, and their industrial/coop experience ranged from 0 to more than 10 years. Table III summarizes students’ experience in
programming, Java experience and industrial experience.}

\input{Tables/Participants}


\subsection{Assignment Content and Format}

\noindent\textcolor{blue}{\textbf{Assignment Design.}} Initially, students are asked to analyze one version of a Java software approved by the instructor to ensure its eligibility based on popularity, besides ensuring it correctly compiles since PMD requires it. The rationale behind giving students the choice of project is to let them choose one that they are comfortable with and fits into their interests.  
For students who do not want to search for a project, they have been given a list that the instructor has already curated (see Table \ref{Table:Project}). We selected these projects as we already know they contain a variety of software defects. 
Then, students are requested to set up and run PMD to analyze the chosen project production code. Students are also given the choice of running either the stand-alone version of the tool, or one of its plugins associated with popular IDEs (Eclipse, IntelliJ), as we want the students to be familiar with the coding environment and reduce the setup overhead. Upon running PMD, students must choose a minimum of 10 warnings, and at least one from each category, if applicable. We enforce the diversification of warnings to ensure a wider exposure to potential issues, varying from design to multithreading, and documentation. It also increases students' learning curve as they cannot reuse their fix to address multiple instances of the same warning. Yet, we allow students to choose the instances they want to address. It implicitly makes students read many warnings, from all categories, which increases the likelihood of incidental learning. Furthermore, letting students choose the code fragments to review increases their confidence in their decision concerning the given warning. 
%, \ie either consider it as a true positive, and provide a code fix or consider it as a false positive, and provide a justification.
 \textcolor{blue}{Finally, the students use \gpt to fix the PMD issues supported by an online questionnaire. For our survey design, we followed the
guidelines proposed by Kitchenham and Pfleeger \cite{kitchenham2008personal}. The survey consisted of \hl{22} questions that are divided
into 2 parts. The first part of the survey includes demographics questions about the participants. In the second part,
we asked about the (1) attitude toward using \gpt to fix PMD issues, (2) perceived \gpt ease of use, and (3) perceived usefulness of ChatGPT. As suggested by Kitchenham and Pfleeger \cite{kitchenham2008personal}, we constructed
the survey uses \hl{6} open-ended questions and \hl{16} multiple-choice questions with an optional \say{Other} category, allowing the respondents to share thoughts not mentioned in the list.}

\noindent\textcolor{blue}{\textbf{Pilot Study.} We  decided to first run a pilot study with two undergraduate students to ensure that the experiment’s instructions were clear. Following the pilot
study, we refined the protocol and questions for assignment interactively. The participants in the pilot study are undergraduate students in Software Engineering. Among others, we learned that prompt engineering is crucial when utilizing ChatGPT, and we
decided to refine survey questions to explore the topic better. Therefore, we reformulated the assignment and excluded the pilot study data from our analysis.}

In a nutshell, students followed these steps:

\begin{enumerate}
    \item Install the PMD.
    \item Run PMD on a project of students' choice and select 10 issues of different types.
    \item Use \gpt to fix the issues.
    \item Report the findings for each issue: (1) the source code, (2) the type of issue, (3) how long it took to check it / fix it, and (4) the code snippet.
    \item Add to the report a concise comment about the experience with \gpt (optional).
    
\end{enumerate}

Submissions artifacts' evaluation was based on 1) assessment of students’ ability to understand the type of issues (concept understanding (RQ1)); 2) assessment of whether students have provided acceptable fixes or proper justification in both cases or accepting or rejecting PMD's recommendation (program analysis and evolution (RQ2)). Students' perception of the code was excluded from the evaluation process, as it can bias the experiment, as students would be filling out the survey arbitrarily, under the pressure of being graded. Also, providing feedback was anonymous and not mandatory to increase the magnitude of PMD usage experience (RQ3). Although feedback was optional, many students have completed it \hl{X}. Figure \hl{X}  depicts an overview of our experiment setup and execution.



\subsection{Assignment Execution}

The assignment was performed over \hl{X} consecutive semesters. \hl{X} students, primarily from computer science (CS) and software engineering (SE) majors, were enrolled during these semesters and completed the assignment. 


\subsection{Data Analysis}
\label{subsec:data-analysis}

    We analyzed the responses to the open-ended question to create a comprehensive high-level list of themes by adopting a thematic analysis approach based on guidelines provided by Cruzes~\etal~\cite{cruzes2011recommended}. Thematic analysis is one of the most used methods in Software Engineering literature~\cite{Silva2016why,alomar2022code,alomar2021refactoring}. This is a technique for identifying and recording patterns (or \say{themes}) within a collection of descriptive labels, which we call \say{codes}. For each response, we proceeded with the analysis using the following steps: \textit{i}) Initial reading of the survey responses; \textit{ii}) Generating initial codes (\ie labels) for each response; \textit{iii}) Translating codes into themes, sub-themes, and higher-order themes; \textit{iv}) Reviewing the themes to find opportunities for merging; \textit{v}) Defining and naming the final themes, and creating a model of higher-order themes and their underlying evidence. The above-mentioned steps were performed independently by two authors. One author performed the labeling of students' comments independently from the other author who was responsible for reviewing the currently drafted themes. \textcolor{black}{By the end of each iteration, the authors met and refined the themes to reach a consensus.}
    \textcolor{black}{It is important to note that the approach is not a single-step process. As the codes were analyzed, some of the first cycle codes were
subsumed by other codes, relabeled, or dropped altogether. As the two authors progressed in the translation to themes, there was some rearrangement, refinement, and data reclassification into
different or new codes. We used the
thematic analysis technique to address RQ3.}
\input{Tables/Project}

\section{Results}
\label{Section:Result}

\subsection{\RQone} \eman{TODO:  add example}

In Tables \ref{Table:pmd-tp-fp-both-a} and \ref{Table:pmd-tp-fp-both-b}, we illustrate PMD rules that are perceived by students.  It is worth noting the diversity of
these warnings/violations, \ie they spread from warnings regarding style, code practice, and documentation, to warnings dealing with design and performance. Thus, upon analyzing students' assignment solutions, we cluster the issues according to the PMD ruleset categories listed in the PMD official documentation\footnote{https://pmd.sourceforge.io}, namely, `Best Practices', `Code Style', `Design', `Documentation', `Error Prone', `Multithreading', `Performance', and `Security'. These categories were captured at different levels of granularity (\eg package, class, method, and attributes). 
%\hl{to be replaced:} Note that we did not report findings related to `Security' category as  students do not seem to select security-related issues. 
%We noticed 
In the rest of this subsection, we provide a more in-depth analysis of these categories and the associated PMD rulesets.

\textbf{Category \#1: Best Practices.} This category refers to the rules that enforce generally accepted best practices vital in an overall assessment of software quality. This category assists students in uncovering code that might violate main design and coding strategies or indicate areas that might consider unnecessarily inefficient or difficult to maintain. Examples of the rules perceived by students as true positives include \texttt{LooseCoupling}, \texttt{SwitchStmtsShouldHaveDefault}, and \texttt{JUnitAssertionsShouldIncludeMessage}. 
%These best practices mainly related to code optimization, which consist of good practices concerning abstraction, JUnit test assertion, 


\textbf{Category \#2: Code Style.}
This category refers to the rules which enforce a specific coding style. Most prominently, brace and naming rules consist of good coding practices regarding code blocks and naming conventions. This can be illustrated briefly by rules \texttt{IfStmtsMustUseBraces} and \texttt{ClassNamingConventions}, which shows that it should be followed by braces even if it is followed only by a single instruction and class names should be in camel case naming conventions to improve naming quality in the  code and reflect the actual purpose of the parameters and variables.

\textbf{Category \#3: Design.} This category refers to the rules which help discover design issues. Students captured design rules that contain best practices concerning overall code structure.  By way of illustration, \texttt{AvoidDeeplyNestedIfStmts} rule  indicates avoiding deeply nested if statements and \texttt{GodClass} shows the violation of single responsibility principles that increases the complexity of the code  (\eg \texttt{CyclomaticComplexity}).


\textbf{Category \#4: Documentation.} This category refers to the rules which are related to code documentation. Documentation is the description, in natural language, of the code-level changes, and such description is crucial as it reveals the developer's rationale behind their coding decisions. \texttt{CommentRequired} rule is a good illustration of this group and shows that students seem to pay
attention to the quality of the code comments.


\textbf{Category \#5: Error Prone.}
This category refers to the rules which detect constructs that are either broken, extremely confusing, or prone to run time errors. One of the key aspects to avoid these issues is readability. If the students refactor the code to be easily read and understood, there is less chance for misunderstandings and coding mistakes, so students spend less time comprehending code. This is exemplified by error-prone-related rules such as \texttt{AvoidDuplicateLiterals} and \texttt{AssignmentInOperand}.

\textbf{Category \#6: Multithreading.} 
This category refers to the rules that flag issues when dealing with multiple threads of execution. For example, PMD recommends  \texttt{AvoidUsingVolatile} to be avoided as the keyword `volatile' is used to fine-tune a Java application and requires the expertise of the Java Memory Model.

\textbf{Category \#7: Performance.}
This category refers to the rules that flag sub-optimal code.
Since performance plays a vital role, students are encouraged to follow best coding standard practices such as \texttt{AvoidArrayLoops} and \texttt{AvoidInstantiatingObjectsInLoops} rules to avoid degrading the performance of the code.  

For our study, \textcolor{black}{we analyzed a total of \hl{1690} rules of students' selected issues} violating \hl{185} distinct PMD rules. As can be seen from Tables \ref{Table:pmd-tp-fp-both-a} and \ref{Table:pmd-tp-fp-both-b}, there are diverse srt of violation chosen by students to be fixed by ChatGPT. While our results are not intended to be generalized, as it requires further experiments with larger sample sizes, our experience shows the success of \gpt in triggering students' critical thinking about the problems outlined in the issues. PMD has successfully attracted them to explore the various types of problems so students can utilize \gpt to code the needed fix for the problem. Moreover, it achieves another goal of our maintenance class, as it trains students to comprehend and act on code that they do not own.  

Looking at the PMD rules, Figure \ref{fig:PMD-relatedcategory} depicts the percentages of PMD rules, clustered by category. As can be seen, the most common PMD ruleset category concerns `Code Style', representing 34.7\% of the issues. This observation is in line with the findings of previous studies describing that most code reviewers look for style conformance when evaluating the quality of code \cite{singh2017evaluating,gousios2015work}. The next most common categories are `Best Practices', `Design', and `Error Prone', representing 19.1\%, 15.9\%, and 12.3\% of the issues, respectively. This might indicate that students have different perspectives on whether developers follow the best practices, improve the architecture design of code, or make code less susceptible to errors. The category `Documentation', `Performance', and `Multithreading' had the least number of issues, which had a ratio of  9.0\%, 6.7\%, and 2.3\%, respectively. 

\begin{tcolorbox}
\textit{\textbf{Summary:} Among the \hl{X} analyzed issues, representing \hl{X} distinct PMD rules.} 
\end{tcolorbox}
%\input{Tables/Participants}

\input{Tables/RQ1}

%\input{Charts/Usefulness}

\input{Charts/Category}
\begin{figure}[t]%[H]
 	\centering
 	\includegraphics[width=1.0\columnwidth]{Images/Boxplot_sigcse.png}
 	\caption{Boxplots of time taken to fix issues, clustered by PMD ruleset categories.}
 	\label{fig:boxplot}
%\vspace{-.4cm}
\end{figure}


\input{Charts/Prompt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\RQtwo}

By looking at Figure \ref{fig:boxplot}, we found issues belonging to the `Design',  `Best Practices', and `Error Prone' categories ($\mu$ = 6.65, $\mu$ = 4.00, and $\mu$ = 4.00, respectively) take more time to be fixed, compared to the other categories. We speculate that these two categories take time to fix as students need to apply techniques to resolve quality flaws or design issues, including code smells (\eg \texttt{GodClass}), and quality attributes (\eg \texttt{CyclomaticComplexity}). This is exemplified in the assignment undertaken by students to resolve the issues. Students refactor the code and optimize the design by performing repackaging, \ie extracting packages and moving the classes between these packages, and merging packages with classes strongly related to each other. The present observations are significant in at least two major respects: (1) improving the quality of packages structure when optimizing cohesion, coupling, and complexity and (2) avoiding increasing the size of the large packages and/or merging packages into larger ones which might have an impact on the following design rules, namely, \texttt{CognitiveComplexity}, \texttt{CyclomaticComplexity}, and \texttt{NPathComplexity}. Further, students might find fixing PMD issues violating best coding practices challenging  when balancing the trade-offs when maintaining efficient code with minimal errors. The other categories take less time to fix when comparing the mean (`Code Style' = 3.56, `Documentation' = 3.40, `Multithreading' = 3.26, `Performance' = 3.22), which might possibly hint at an easy resolution of the reported issues or warnings.

We speculate that design issues take significantly longer to be resolved because of substantial modifications need to be made for certain design issues such as \texttt{GodClass}. While \gpt demonstrates its capability to propose beneficial fixes by analyzing the code segments, it has limitations in grasping the larger context in which these segments are utilized. Due to this limitation, there have been instances where ChatGPT makes suggestions based on misunderstandings or false assumptions about the code. In contrast, human programmers possess the knowledge and understanding necessary to consider such broader contextual information. 

\begin{tcolorbox}
\textit{\textbf{Summary:} `Design' PMD ruleset category takes longer to resolve. Unlike other PMD category, this requires going beyond one or few instructions, and ChatGPT has a limited understanding of the broader
context and entirety of the codebase.}   
\end{tcolorbox}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\RQthree}
\input{Charts/ChatGPT_usage}
Figure \ref{fig:ChatGPT usage} shows students' attitude toward utilizing ChatGPT in terms of various aspects: (1) the ChatGPT's capability to resolve bugs, (2) the possibility for ChatGPT's to introduce additional violations through PMD, (3) the potential for ChatGPT to introduce compilation errors, (4) the frequency of interaction with ChatGPT for bug-fixing purposes, and (5) the effectiveness of ChatGPT in resolving bugs. When we asked students, \say{Was ChatGPT able to fix the buggy code?}, 84.4\% of the students indicated that ChatGPT is able to fix bugs, but 15.6\% of the students responded negatively. As for the potential to introduce additional violations through PMD, the majority of students (85.5\%) mentioned that ChatGPT does not contain other errors detected by PMD, but a few indicated otherwise. Regarding the introduction of compilation errors, 87.7\% of the students revealed there is no compilation errors, while 12.3\% of students experienced it. In terms of the frequency of the usage and interaction with ChatGPT before finding (or not) a fix to the buggy code, 51.8\% used it once, 22\% used it twice. The remaining students (26.2\%) used \gpt between three and more than five times. Lastly, concerning usefulness of ChatGPT, the vast majority of students (96.8\%) stated affirmatively, acknowledging that \gpt is indeed useful.

Further, as shown in Figure \ref{fig:prompt}, we report how students use \gpt to fix the buggy code. The majority of students (68.6\%) communicated that they were copy-paste the buggy code fragment along with error description. 27.7\% of students revealed that they only copy-paste the buggy code fragments. 20.6\% of students mentioned that they copy-paste the buggy code fragment and added textual description of how to fix it. A few students reported that they show pairs of buggy and fixed code fragments and asked \gpt to do similar for the given buggy code. Besides these activities, 2.9\% of the students mentioned in the \say{other} option: \say{\textit{asking ChatGPT that the PMD violation still remained when it could not fix the code}}, \say{\textit{asking ChatGPT how to fix the error in general before copy pasting the offending code}}, \say{\textit{prompted ChatGPT with the actual line that was causing the error and asked it if there was something specific in the code segment that could be optimized}}, \say{\textit{asked ChatGPT to provide an example of how a similar situation could be fixed}}, and \say{\textit{ChatGPT says this is a false positive and is descriptive of what the variable is representing and I agree with it}}. We conjecture that students might opt for different prompt engineering due the variability of ChatGPT's responses. It
has been proven by previous studies that \gpt is susceptible to hallucination when they asked the AI about code semantic structures \cite{ma2023scope,white2023chatgpt}. 
%\say{\textit{False positive - ChatGPT was not needed.}}. 

In Table~\ref{Table:example}, we report the main thoughts, comments, and suggestions about the overall impression of the usefulness, usability, functionality, and recommendation of the ChatGPT, in accordance with the conducted labeling. The table also presents samples of the students' comments to illustrate their impressions of each theme.

\textbf{Usefulness.} Generally, the respondents found the \gpt to be useful in regard to five main aspects: automation, awareness, experience, quality, and scope. A group of students commented that the ChatGPT's ability to automatically fix bugs, its affordability, capacity for automating tedious debugging and bugfixing processes, and ability to deliver precise and thorough responses . Nearly \hl{X} of the students commented that \gpt is useful as it gave explanations as to what the problem was and the suggestion to fix it.  Further,  \hl{X} of students commented that it is a nice application and provides a good learning experience especially for those who are begineers in software development and maintenance. A few students (\hl{X}) revealed that the \gpt was fast in terms of analyzing simple code, but not for  identifying larger issues such as \texttt{GodClass}, and \texttt{DataClass}. \hl{X} of students communicated that detecting the issues assists in increasing its \textit{readability}, which helps improve overall code quality.
\input{Tables/Comment}

\textbf{Usability.}  Based on the feedback provided by the students, the key areas in usability related to documentation, ease of use, explainability, and user interface. \hl{X} of the students pointed out the tool is easy to use, has a user-friendly interface, and explains how it preformed each bugfix and how to avoid that issue in the future. Other comments also stated using these LLMs requires to carefully adjust the model's output. It lacks originality and might give biased output. 

\textbf{Functionality.} According to the students' feedback about the tool's functional features, \hl{X} of the students' comments \textcolor{black}{appreciate ChatGPT's correction, detection and debugging functionality and are satisfied with various aspects of the tool’s operation}, and how this feature helps in better understanding of bad programming practices in real-world scenarios. Additionally, the students commented on their ability to practice a variety of strategies to remove issues. 

\textbf{Recommendation.} From the students' feedback, we have also extracted suggestions to improve the LLMs. \hl{X} of the students' comments show a couple of suggested changes as a recommendation to be made to the tool's operation. We found out the students pointed out some of the recommendations related to accuracy, context, prompt, resolution and verification. Students commented  that it is undeniable that ChatGPT's capabilities have the potential to transform the programming process for developers. With its remarkable ability to generate multiple solutions to a problem and adapt to a developer's preferred approach, \gpt hampers creativity of people and is poised to revolutionize the way developers approach coding in the future. Other students felt that \gpt could fix small errors quickly and explained them well given the PMD rules. But when the errors got a little complex, it is difficult to let \gpt know of the whole context of the project so the proposed solutions can be wrong at times. Therefore, it must be utilized carefully and its results must be confirmed and verified by other sources of information. The fact that ChatGPT's replies are determined by the prompt it gets and the data it was trained on could be a drawback as The quality of its responses are 
highly dependent on the quality of the prompts. Its solutions might not always be precise or appropriate for the particular activity or topic. Students also mentioned that \gpt is helpful in most situations. However, it struggles to solve issues without context. For example, \gpt might find the code comprehensive and easy to read but when students mention the problem with the code, it then recognizes the issue. The more detail description is, the more specific and accurate solution is made by ChatGPT. However, some code which is a large file and issue is needed to check for all the file is predicament for \gpt to deal with.







 
\begin{tcolorbox}
\textit{\textbf{Summary:} Overall, students exhibit some level of skepticism towards using \gpt to find and fix bugs. However, the assignment helps in cultivating students' analytical and critical thinking skills while they engage in the debugging process. Our study sheds light on the limitations  of  ChatGPT  in identifying and resolving bugs. It highlights the importance  of  incorporating  other  traditional static analysis  tools  and  techniques  to improve the accuracy and efficiency of their predictions. Furthermore, the involvement of a human-in-the-loop, capable of comprehending code, can be highly valuable and desirable.} 
\end{tcolorbox}

%don't entirely trust \gpt, but the assignment  develops students' critical and analytical skills during the debugging process


%\vspace{-.6cm}
\section{Reflection}
\label{Section:Reflection}

This section provides the lessons learned from both educator and student perspectives. \eman{The section needs to be revised to ensure its educational soundness.}

\noindent\textbf{Lesson \#1:  \textit{Develop complementary  assignments.}}
\gpt identified what each of the PMD violations was and attempted to fix them. In some cases, it would cause the problem to vanish from the PMD analyzer completely. In other cases, although the issue was fixed, the PMD analyzer would still detect the problem as present, even when the file was rescanned with the edited code included. \gpt re-edits the code when prompted; sometimes, it will improve its response. However, when given the same prompt multiple times, it will generate the same response without alteration after many attempts. Therefore, the students can use \gpt as
a complementary tool alongside traditional static analysis tools
 to improve the efficiency of their software development process. 

 
\noindent\textbf{Lesson \#2:  \textit{Limited understanding of the broader context of the codebase.}} While \gpt was  informative about giving context and definitions of errors and could  provide recommendations specific to the PMD tool,  it has a limited understanding of the broader context and entirety of the codebase, which might lead to miss dependencies and co-dependencies. Due to this limitation, there have been instances where ChatGPT makes suggestions based on misunderstandings or false assumptions about the code.  %Also, \gpt often supposed the code has the issue, so it is hard for it to identify the true or false of the issue later correctly. The student must first identify the PMD's checking results as true positive.
 Also, in some cases, \gpt cannot fix the code with best practices; its solution will increase the cyclomatic complexity, probably due to the lack of context in the code snippets. This observation is in line with previous studies \cite{christakis2016developers,johnson2013don} finding that bad warning messages and no suggested fixes are one of the pain points reported by industrial software developers when using program analyzers. 

 \noindent\textbf{Lesson \#3:  \textit{Verify ChatGPT's responses with human expertise.}} While \gpt can provide some help in debugging, it should not be relied on as the only debugging tool. As shown in Table \ref{Table:example}, \gpt is perfect as a code companion but not a replacement. The reason for this is that \gpt cannot find the context of the applications of code. Having a human-in-the-loop who can understand the applications is much more desirable. Thus, experienced developers and specialized debugging tools remain essential for thorough and effective debugging.


\noindent\textbf{Lesson \#4:  \textit{Automate the debugging and bugfixing process.}} \gpt is an effective tool for programmers seeking assistance. Still, providing clear and detailed questions is essential to get the most accurate and helpful responses. It has helped students debug and clarify what each code segment did and explained how it performed each bugfix. Thus, the process is significantly shortened. Yet, in a few cases, it required some experimentation before coming up with a set of questions to accomplish the task.  
 Additionally, it suggested changes that caused compiler errors, \eg renaming a variable in a field declaration or fixing a different issue in the code rather than the one given to analyze. Further, \gpt tends to view stylistic or best practice PMD-related issues as not problematic and is too light-handed in explaining the potential issues with stylistic/best practice problems in source code. In the real world, this can lead to a student developing bad coding habits, ultimately detrimental to the productivity of the individual and the team they belong to. some of the flaws were observed with inexplicable fixes or suggestions. 



\noindent\textbf{Lesson \#5:  \textit{Improve ChatGPT's accuracy and effectiveness.}} \gpt was useful in resolving a few PMD rule violations and provided good recommendations for resolving them.  In a few cases, however, it cannot determine as a PMD rule violation even though providing the code snippet with context. For a few violations, it answered as 'may,' providing it satisfying given conditions since it only provided the code snippet and not the surrounding code. We believe if the \gpt is trained properly for the specific ruleset, it can be used for clearing out PMD rule violations quicker. Yet, one cannot highly rely only on \gpt, some level of understanding and knowledge is required by the developer to make the appropriate correction. Additionally, it sometimes generates code that produces compile errors. 

\noindent\textbf{Lesson \#6:  \textit{Handle complex code and errors.}} The effectiveness of \gpt is closely tied to the quality of its training data set. As per students' comments, \gpt provides high-level and valuable suggestions about the bugs. For instance, it is useful in fixing non-pressing matters such as code style, adding comments, making the if-statements more logical, etc. On the other hand, it would sometimes misunderstand the error the student was trying to indicate or would be confused by the fact that the input gave it a code excerpt rather than the full code, which was too large to provide. Its corrections sometimes also misunderstood the purpose of an excerpt and would slightly alter the logic. So,  the more complex the given code input, the more likely the code output will not work properly.

\noindent\textbf{Lesson \#7:  \textit{\eman{Mohamed: here is your point}\hl{train students not to accept everything from ChatGPT.}}}

%\vspace{-.6cm}
\section{Reflection}
\label{Section:Reflection}

This section provides the lessons learned from both educator and student perspectives. \eman{The section needs to be revised to ensure its educational soundness.}

\noindent\textbf{Lesson \#1:  \textit{Develop complementary  assignments.}}
\gpt identified what each of the PMD violations was and attempted to fix them. In some cases, it would cause the problem to vanish from the PMD analyzer completely. In other cases, although the issue was fixed, the PMD analyzer would still detect the problem as present, even when the file was rescanned with the edited code included. \gpt re-edits the code when prompted; sometimes, it will improve its response. However, when given the same prompt multiple times, it will generate the same response without alteration after many attempts. Therefore, the students can use \gpt as
a complementary tool alongside traditional static analysis tools
 to improve the efficiency of their software development process. 

 
\noindent\textbf{Lesson \#2:  \textit{Limited understanding of the broader context of the codebase.}} While \gpt was  informative about giving context and definitions of errors and could  provide recommendations specific to the PMD tool,  it has a limited understanding of the broader context and entirety of the codebase, which might lead to miss dependencies and co-dependencies. Due to this limitation, there have been instances where ChatGPT makes suggestions based on misunderstandings or false assumptions about the code.  %Also, \gpt often supposed the code has the issue, so it is hard for it to identify the true or false of the issue later correctly. The student must first identify the PMD's checking results as true positive.
 Also, in some cases, \gpt cannot fix the code with best practices; its solution will increase the cyclomatic complexity, probably due to the lack of context in the code snippets. This observation is in line with previous studies \cite{christakis2016developers,johnson2013don} finding that bad warning messages and no suggested fixes are one of the pain points reported by industrial software developers when using program analyzers. 

 \noindent\textbf{Lesson \#3:  \textit{Verify ChatGPT's responses with human expertise.}} While \gpt can provide some help in debugging, it should not be relied on as the only debugging tool. As shown in Table \ref{Table:example}, \gpt is perfect as a code companion but not a replacement. The reason for this is that \gpt cannot find the context of the applications of code. Having a human-in-the-loop who can understand the applications is much more desirable. Thus, experienced developers and specialized debugging tools remain essential for thorough and effective debugging.


\noindent\textbf{Lesson \#4:  \textit{Automate the debugging and bugfixing process.}} \gpt is an effective tool for programmers seeking assistance. Still, providing clear and detailed questions is essential to get the most accurate and helpful responses. It has helped students debug and clarify what each code segment did and explained how it performed each bugfix. Thus, the process is significantly shortened. Yet, in a few cases, it required some experimentation before coming up with a set of questions to accomplish the task.  
 Additionally, it suggested changes that caused compiler errors, \eg renaming a variable in a field declaration or fixing a different issue in the code rather than the one given to analyze. Further, \gpt tends to view stylistic or best practice PMD-related issues as not problematic and is too light-handed in explaining the potential issues with stylistic/best practice problems in source code. In the real world, this can lead to a student developing bad coding habits, ultimately detrimental to the productivity of the individual and the team they belong to. some of the flaws were observed with inexplicable fixes or suggestions. 



\noindent\textbf{Lesson \#5:  \textit{Improve ChatGPT's accuracy and effectiveness.}} \gpt was useful in resolving a few PMD rule violations and provided good recommendations for resolving them.  In a few cases, however, it cannot determine as a PMD rule violation even though providing the code snippet with context. For a few violations, it answered as 'may,' providing it satisfying given conditions since it only provided the code snippet and not the surrounding code. We believe if the \gpt is trained properly for the specific ruleset, it can be used for clearing out PMD rule violations quicker. Yet, one cannot highly rely only on \gpt, some level of understanding and knowledge is required by the developer to make the appropriate correction. Additionally, it sometimes generates code that produces compile errors. 

\noindent\textbf{Lesson \#6:  \textit{Handle complex code and errors.}} The effectiveness of \gpt is closely tied to the quality of its training data set. As per students' comments, \gpt provides high-level and valuable suggestions about the bugs. For instance, it is useful in fixing non-pressing matters such as code style, adding comments, making the if-statements more logical, etc. On the other hand, it would sometimes misunderstand the error the student was trying to indicate or would be confused by the fact that the input gave it a code excerpt rather than the full code, which was too large to provide. Its corrections sometimes also misunderstood the purpose of an excerpt and would slightly alter the logic. So,  the more complex the given code input, the more likely the code output will not work properly.

\noindent\textbf{Lesson \#7:  \textit{\eman{Mohamed: here is your point}\hl{train students not to accept everything from ChatGPT.}}}


